Quantitative Information Flow as Safety and Liveness Hyperproperties

We employ Clarkson and Schneider's "hyperproperties" to classify various verification problems of quantitative information flow. The results of this paper unify and extend the previous results on the hardness of checking and inferring quantitative information flow. In particular, we identify a subclass of liveness hyperproperties, which we call "k-observable hyperproperties", that can be checked relative to a reachability oracle via self composition.

==> eptcsdata.tex <==
\providecommand{\firstpage}{77}
\providecommand{\publicationstatus}{M. Massink and H. Wiklicky (Eds.):Workshop on Quantitative\\
Aspects of Programming Languages and Systems 2012 (QAPL 2012)\\
EPTCS 85, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.85.6}{10.4204/EPTCS.85.6}}

